LIGHTYEAR: Using Modularity to Scale BGP Control Plane Verification

Current network control plane verification tools cannot scale to large networks, because of the complexity of jointly reasoning about the behaviors of all nodes in the network. In this paper we present a modular approach to control plane verification, whereby end-to-end network properties are verified via a set of purely local checks on individual nodes and edges. The approach targets the verification of safety properties for BGP configurations and provides guarantees in the face of both arbitrary external route announcements from neighbors and arbitrary node/link failures. We have proven the approach correct and also implemented it in a tool called Lightyear. Experimental results show that Lightyear scales dramatically better than prior control plane verifiers. Further, we have used Lightyear to verify three properties of the wide area network of a major cloud provider, containing hundreds of routers and tens of thousands of edges. To our knowledge no prior tool has been demonstrated to provide such guarantees at that scale. Finally, in addition to the scaling benefits, our modular approach to verification makes it easy to localize the causes of configuration errors and to support incremental re-verification as configurations are updated.

==> figures/tables/univeristy-properties-table.tex <==

\begin{table*}
    \begin{tabular}{|l|llp{2.8in}|}
    \hline
        \textbf{Type}           & \textbf{Locations ($l$)}      &    \textbf{Logical Formula ($I_l$)} & \textbf{Description}    \\ \hline
        \makecell[l]{End-to-end \\ Property} &  \makecell[l]{Edges to ISP \\ R $\rightarrow$ P} & $\textsc{Prefix}(r) \in \textsc{UniPrefixes}$ & 
        \textit{University routers only send prefixes for its owned address blocks} \\ \hline
       
        \multirow{2}{*}{\begin{tabular}{l} Initial \\ Network \\ Invariants \end{tabular}} & \makecell[l]{Edges to ISP \\ R $\rightarrow$ P} & $\textsc{Prefix}(r) \in \textsc{UniPrefixes}$ & 
        \textit{University routers only send prefixes for its owned address blocks} \\ \cline{2-4}
        & \makecell[l]{Other} & True & \textit{Other locations are unconstrained} \\ \hline
        \multirow{3}{*}{\begin{tabular}{l} Refined \\ Network \\  Invariants \end{tabular}} & \makecell[l]{Edges to ISP \\ R $\rightarrow$ P} & $\textsc{Prefix}(r) \in \textsc{UniPrefixes}$ & \textit{University routers only send prefixes for its owned address blocks} \\ \cline{2-4}
        & \makecell[l]{Edges from external \\ $P \rightarrow R$} & True & \textit{Routes from external neighbors are unconstrained} \\ \cline{2-4}
        & \makecell[l]{Other} & $\comm{r}\ \cap \textsc{ SComms} = \emptyset$ & \textit{Routes at other locations inside network are not tagged with specific communities} \\ \hline
    \end{tabular}
    \caption{The end-to-end property and network invariants needed to verify that the university only advertises its own aggregated networks. Both the initial guess and the refined invariants are shown.}
    \label{tab:univ-invariants}
\end{table*}
